Excited doubly heavy baryons production via top-quark decays

Within the framework of NRQCD, we calculate the production of excited doubly heavy baryons $\Xi_{bQ}$ through the semi-inclusive production process $t\rightarrow \langle bQ\rangle[n]\rightarrow \Xi_{bQ}+ \bar {Q} + W^+ $, where $Q= b$ or $c$ quark. The intermediate diquark state $\langle bQ\rangle[n]$ is in the excited $P$-wave state, including $[^1P_1]$ and $[^3P_J]$ ($J=$0, 1 or 2) in both color antitriplet state $\mathbf{\mathbf{\overline 3}}$ and color sixtuplet state $\mathbf{6}$, that is, $\langle bc\rangle[^{1}P_{1}]_{\mathbf{\overline 3}/ \mathbf{6}}$, $\langle bc\rangle[^{3}P_{J}]_{\mathbf{\overline 3}/ \mathbf{6}}$, $\langle bb\rangle[^{1}P_{1}]_{\mathbf{\overline 3}}$, and $\langle bb\rangle[^{3}P_{J}]_{\mathbf{6}}$. We find that the contributions from the P-wave states are about one order lower than the S-wave contributions, and this conclusion is consistent with others. We also analyze the invariant mass and angle differential distributions, and the theoretical uncertainty from the mass parameters and the renormalization scale. Finally, we can expect that about $1.14 \times10^{3-5}$ events of excited $\Xi_{bc}$ and $2.47 \times10^{1-3}$ events of excited $\Xi_{bb}$ can be produced per year at the LHC or HL-LHC with $\mathcal{L}$ =$10^{34-36}~\rm{cm}^{-2}~\rm{s}^{-1}$.

==> pst-tools.tex <==
%% $Id: pst-tools.tex 674 2017-12-02 22:04:53Z herbert $
%%
%% This is file `pst-tools.tex',
%%
%% IMPORTANT NOTICE:
%%
%% Package `pst-tools.tex'
%%
%% Herbert Voss <hvoss@tug.org>
%%
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN archives
%% in directory macros/latex/base/lppl.txt.
%%
%% DESCRIPTION:
%%   `pst-tools' is a PSTricks package for helper functions
%%
%%
\csname PSTtoolsLoaded\endcsname
\let\PSTtoolsLoaded\endinput

\ifx\PSTricksLoaded\endinput\else\input pstricks.tex\fi
\ifx\PSTXKeyLoaded\endinput\else \input pst-xkey.tex \fi
%
\edef\PstAtCode{\the\catcode`\@} \catcode`\@=11\relax
% interface to the `xkeyval' package
\pst@addfams{pst-tools}
%
\def\fileversion{0.09b}
\def\filedate{2017/12/03}
\message{`PST-tools' v\fileversion, \filedate\space (hv)}
%
\define@key[psset]{pst-tools}{decimalSeparator}[.]{\def\psk@decimalSeparator{#1}}%
\define@boolkey[psset]{pst-tools}[Pst@]{comma}[true]{%
  \ifPst@comma\def\psk@decimalSeparator{,}\else\def\psk@decimalSeparator{.}\fi}
\define@boolkey[psset]{pst-tools}[Pst@]{trimSpaces}[true]{}
\define@key[psset]{pst-tools}{xShift}[0]{\def\psk@xShift{#1}}
\define@key[psset]{pst-tools}{yShift}[0]{\def\psk@yShift{#1}}
\define@key[psset]{pst-tools}{postString}[{}]{\def\psk@postString{#1}}
\define@key[psset]{pst-tools}{VarName}[]{\def\psk@VarName{#1 }}
\define@key[psset]{pst-tools}{PSfont}[NimbusRomNo9L-Regu]{\def\psk@PSfont{/#1 }}
\define@key[psset]{pst-tools}{valuewidth}[10]{\pst@getint{#1}\psk@valuewidth }
\define@key[psset]{pst-tools}{fontscale}[10]{\pst@checknum{#1}\psk@fontscale }
\define@key[psset]{pst-tools}{decimals}[-1]{\pst@getint{#1}\psk@decimals }
\psset[pst-tools]{PSfont=NimbusRomNo9L-Regu,fontscale=10,valuewidth=10,decimals=-1,
                  xShift=0,yShift=0,trimSpaces=false,postString={},VarName={},
                  comma=false,decimalSeparator=.}
%
\def\txG{ true setglobal globaldict begin }
\def\etxG{ end false setglobal }
%
\newpsstyle{mmpaper}{subgriddiv=5,gridlabels=0,gridwidth=1pt,gridcolor=orange,subgridwidth=0.1pt,subgridcolor=orange!90}
%
\def\psPrintValue{\pst@object{psPrintValue}}
\def\psPrintValue@i#1{\expandafter\psPrintValue@ii#1,,\@nil}
\def\psPrintValue@ii#1,#2,#3\@nil{%  #1,#2 only for algebraic code
  \begin@SpecialObj
  \addto@pscode{  
     gsave \psk@PSfont findfont \psk@fontscale scalefont setfont 
     \ifPst@algebraic 
       /x #1 def 
       /Func (#2) tx@AlgToPs begin AlgToPs end cvx def 
       Func 
     \else #1 \fi
     \ifx\relax\psk@VarName\relax\else dup \txG 10 string cvs /\psk@VarName\space exch def \etxG \fi
     \psk@decimals -1 gt { 10 \psk@decimals exp dup 3 1 roll mul cvi exch div } if
     \psk@valuewidth string cvs %/Output exch def % save output
%/concatstringarray{  %  [(a) (b) ... (z)] --> (ab...z)  20100422
     \ifx\relax\psk@postString\relax\else [ exch (\psk@postString) ] concatstringarray \fi
     \ifPst@trimSpaces rightTrim \fi
     \ifPst@comma dot2comma \fi        % do we have to change dot to comma
     \psk@xShift\space \psk@yShift\space moveto  %Output 
     show grestore
  }%
  \end@SpecialObj%
}

\define@boolkey[psset]{pst-tools}[Pst@]{round}[true]{}%
\define@boolkey[psset]{pst-tools}[Pst@]{science}[true]{%
  \ifPst@science\def\psk@Scin{true }\else\def\psk@Scin{false }\fi}
\psset[pst-tools]{science=false,round=false}
%
\def\psPrintValueNew{\pst@object{psPrintValueNew}}
\def\psPrintValueNew@i#1{\expandafter\psPrintValueNew@ii#1,,!!}
\def\psPrintValueNew@ii#1,#2,#3!!{%  #1,#2 only for algebraic code
  \begin@SpecialObj
  \addto@pscode{  %		thanks to Buddy Ledger
     /mfont { \psk@PSfont findfont \psk@fontscale scalefont setfont } bind def
     /mfontexp { \psk@PSfont findfont \psk@fontscale 1.2 div scalefont setfont } bind def
     /s1 { /StandardSymL findfont \psk@fontscale scalefont setfont } bind def
     \ifPst@algebraic 
        /x #1 def
        /Func (#2) tx@AlgToPs begin AlgToPs end cvx def 
        Func  
     \else #1 \fi
     /value exch def
     \psk@Scin {
       value 0 ne { value log floor cvi /expon exch def }{ /expon 0 def } ifelse
       value 10 expon exp div 
       \psk@decimals -1 gt { 10  \psk@decimals exp dup 3 1 roll mul 
         \ifPst@round round \else cvi \fi  exch div } if
       \psk@decimals 0 eq { cvi } if /numb exch def
       expon \psk@valuewidth string cvs /expon exch def
       numb \psk@valuewidth string cvs 
       \ifPst@comma dot2comma \fi  % do we have to change dot to comma
       /Output exch def
       /txspc \psk@fontscale 4 div def
       \psk@xShift\space 0 moveto mfont Output show
       txspc 0 rmoveto s1 (\string\264) show
       txspc 0 rmoveto mfont (10) show
       txspc 2 div txspc 1.5 mul rmoveto mfontexp expon show }
     { value
       \psk@decimals -1 gt { 10 \psk@decimals exp dup 3 1 roll mul 
         \ifPst@round round \else cvi \fi exch div } if
       \psk@decimals 0 eq { cvi } if %inserted to handle decimals=0
       \psk@valuewidth string cvs 
       \ifPst@comma dot2comma \fi         % do we have to change dot to comma
       \psk@xShift\space 0 moveto mfont %Output 
       show
     } ifelse
  }%
  \end@SpecialObj
}
%
\def\psRegisterList#1#2{%
  \@namedef{#1}##1{\@nameuse{#1##1}}%
  \pst@cnto=1
  \@for\pst@tempA:=#2\do{%
    \edef\pst@tempB{\@namedef{#1\the\pst@cnto}{\pst@tempA}}%	
    \pst@tempB
    \advance\pst@cnto by 1
  }%
}

\catcode`\@=\PstAtCode\relax
%
%% END: pst-tools.tex
\endinput
%

